Towards Understanding Adversarial Transferability in Federated Learning

We investigate a specific security risk in FL: a group of malicious clients has impacted the model during training by disguising their identities and acting as benign clients but later switching to an adversarial role. They use their data, which was part of the training set, to train a substitute model and conduct transferable adversarial attacks against the federated model. This type of attack is subtle and hard to detect because these clients initially appear to be benign. The key question we address is: How robust is the FL system to such covert attacks, especially compared to traditional centralized learning systems? We empirically show that the proposed attack imposes a high security risk to current FL systems. By using only 3\% of the client's data, we achieve the highest attack rate of over 80\%. To further offer a full understanding of the challenges the FL system faces in transferable attacks, we provide a comprehensive analysis over the transfer robustness of FL across a spectrum of configurations. Surprisingly, FL systems show a higher level of robustness than their centralized counterparts, especially when both systems are equally good at handling regular, non-malicious data. We attribute this increased robustness to two main factors: 1) Decentralized Data Training: Each client trains the model on its own data, reducing the overall impact of any single malicious client. 2) Model Update Averaging: The updates from each client are averaged together, further diluting any malicious alterations. Both practical experiments and theoretical analysis support our conclusions. This research not only sheds light on the resilience of FL systems against hidden attacks but also raises important considerations for their future application and development.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
The ever-growing usage of mobile devices such as smartphones and tablets leads to an explosive amount of distributed data collected from user end. Such private and sensitive data, if can be fully utilized, will greatly improve the power of more intelligent systems. 
Federated learning (FL) provides a solution to decentralized learning by training quality models through local updates and parameter aggregation \cite{mcmahan2017communication}. 
A FL system maintains a loose federation of participated clients and a centralized server that holds no data but the aggregated model. During training, the central server distributes the global model to a random subset of participants where they update the model with the private data locally and submit the updated model back to the server 
% which are aggregated 
for aggregation
(\eg, average) at each round. 
By design, the system has no visibility of the local data, 
% of participants, 
allowing it to benefit from a wide range of private data while maintaining participant privacy, 
% while 
and the averaging provides an efficient way to leverage the updated parameters compared with distributed SGD.

Despite the fact that FL protects privacy, the loose organization and its invisibility to local data makes it more vulnerable to various attacks including data poisoning \cite{huang2011adversarial}, model poisoning (backdoor attack) \cite{bhagoji2019analyzing, bagdasaryan2020backdoor}, free-riders attack \cite{lin2019free} and various reconstruction attack that leaks the data and privacy of individual participants \cite{geiping2020inverting, zhu2019deep}. 
% To reduce the security breach in federated learning, numerous researchers have strived to develop a robust method resistant to these attacks. 
% Various anomaly detection based methods have been proposed to prevent possible poisoning attacks such as Byzantine-tolerant aggregation \cite{yin2018byzantine}, clustering-based selection \cite{shen2016auror} and anomaly detection in spectral domain \cite{li2020learning}. Reputation is introduced to prevent free-rider \cite{xu2020reputation} and differential privacy techniques are leveraged to preserve the privacy against GANs-based reconstruction attacks \cite{augenstein2019generative, hao2019towards}. 
Another line of FL security research focuses 
on the attack 
during inference, i.e., the adversarial attack \cite{biggio2013evasion, szegedy2013intriguing}. Same as any other deep learning application, 
federated systems are also found vulnerable to the adversarial examples carefully crafted to deceive the model \cite{zizzo2020fat}. 
FAT first discusses the possibility of attacking the federated model with adversarial examples and the interplay of adversarial training with FL \cite{zizzo2020fat}. 
What is following is a line of research proposing a more robust FL method tailored to defend the adversarial examples \cite{zhou2020adversarial, reisizadeh2020robust, hong2021federated}. 
Despite great progress made, the community mainly focuses on a %idealized seems to be a very strong word
white-box setting where the attacker gets full access to the various aspects of the target model such as the gradient and the output of the model. 
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/main.pdf}
%     \vspace{-10pt}
%     \caption{The practical setting of our interest: some clients are disguised as normal clients and participate the training process of a FL system regularly, but later contribute the \emph{data} to train a malicious model
%     for attacking the trained FL system, 
%     because the local weights can be secured through 
%     the FL software.
%     This paper studies the possibility 
%     of such attack across different configurations of the FL system.
%     }
%     \label{fig:main}
% \end{figure}
However, in most real-world scenarios where FL system, \eg, Gboard \cite{hard2018federated}, is trained and deployed, adversary have no access to any knowledge of the model or the full training set.

Different from the above two settings, 
we notice that 
FL is naturally raising another security and robustness challenge:
during the training, 
the malicious client can disguise to be a benign one to 
contribute regularly to the update of the model parameters, 
and only reveal its adversary identity after the training. 
Thus, the client naturally obtains a subset of the data
used to train the FL model,  
and has the potential to exploit this slice of data for adversarial attacks. 
While most of the federated application poses no criteria for eliminating the hostile participants \cite{hard2018federated}, even if there are selection mechanisms (\eg Krum for defending backdoor attack) \cite{fang2020local, li2020learning, bagdasaryan2020backdoor}, the attacker undoubtedly escapes from it since no hostile actions are performed during training. The attacker, after acquiring the data, can train a surrogate model to perform the transfer-based black-box attack.

% Imagine an adversary who wants to manipulate the output of an federated-trained autopilot system for some hostile purposes, \eg hijack for ransom on the highway. If the autopilot system equips models trained in an centralized manner, the attacker will have to perform query-based black-box or transfer-based black-box attack. Query-based attack requires multiple queries which leads to significantly high cost and the risk of  being detected by the system. Transfer-based attack, on the other hand, requires the full original training set or a similar training set which is much more difficult to steal from the server provider or laborsome to collect and annotate.  In the case where FL system is deployed, however, the autopilot system would be much more vulnerable to the attack since the distributed properties makes the training data much more easier to access than that in a centralized training. Now, the adversary can easily access part of the training data if he participates in the federated training. The adversary might also mange to access the data from multiple cars through hacking or stealing. While most of the federated application poses no criteria for eliminating the hostile participants \cite{hard2018federated}, even if there are selection mechanisms (\eg Krum for defending backdoor attack) \cite{fang2020local, li2020learning, bagdasaryan2020backdoor}, the attack undoubtedly escapes from it since no hostile actions are done during training. The attack, after acquiring the data, can train a surrogate model to perform the black-box attack.

In this paper, we take the first step to explore this practical perspective of robustness in FL. Stemming from the above-discussed scenarios, we propose a simple yet practical assumption: 
the attacker possesses some but a limited amount of the users' data but no knowledge about the target model or the full training set. 
To better understand and evaluate the robustness of current FL systems and provide implications for future research to improve security in this regard, we conduct investigations on the adversarial transferability under a spectrum of practical FL settings. 
First, we establish baseline models with ResNet50 on CIFAR10 to provide a preliminary understanding about the robustness of FL under a white-box attack. Then we evaluate the transferability of adversarial examples generated from different source models to attack a federated-trained model. We further investigate two properties of FL, namely the decentralized training and the averaging operation, and their correlation with federated robustness. To provide a comprehensive evaluation in practical aspect, we take into account the attack timing, the architecture and different aggregation methods in our experiments. We have the following findings:
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item We find that, 
    while there is indeed security challenges of this setting (\ie the malicious clients can attack the federated model after the training through transferable adversarial examples), 
    the federated model is more robust under white-box attack compared with its centralized-trained counterpart when their accuracy on clean images are comparable.
    \item We investigate the transferability of adversarial examples generated from models trained by various number of users' data. We observe that, without any elaborated techniques such as dataset synthesis \cite{papernot2017practical} or attention \cite{wu2020boosting},
    a regularly trained source model with only limited users' data can perform transfer attack. With ResNet50 on CIFAR10 datatset, we achieve an transfer rate of over 60\% with only 10\% of the total clients and an transfer rate of almost 90\% with 20\%. With strong augmentation, source model can have a transfer rate of almost 70\%  and 80\% with only 5\% and 7\% of 
    % the total 
    users.
    \item We investigate two intrinsic properties of the FL, namely the property of distributed training and the averaging operation and discover that both heterogeneity and dispersion degree of the decentralized data as well as the averaging operations can significantly decreases the transfer rate of transfer-based black-box attack. We provide theoretical support to further analyze the two observations.  
\end{itemize}

==> sections/preliminary.tex <==
\section{Background}
\label{sec:background}
To better present our investigation and findings, we first introduce the background including the definition of adversarial robustness, current research on the various security problems of FL and their defense, and finally the definition of our proposed attack setting.
% \hwc{maybe comment this paragraph out for space}

\subsection{Adversarial Robustness}
The adversarial robustness of a model is
usually 
defined as the model's ability to predict consistently in the presence of small changes in the input. 
Intuitively, if the changes to the image are so tiny that they are imperceptible to humans, these perturbations will not alter the prediction.
% of the model. 
% This robustness to small changes in the input can be formally described as: 
Formally, 
given a well trained classifier $f$ and image-label pairs $(x, y)$ on which the model correctly classifies $f(x) = y$, $f$ is defined to be $\epsilon$-robust with respect to distance metric $d(\dot, \dot)$ if
\begin{equation}
   \mathbb{E}_{(x, y)} \min_{x':d(x', x) \le \epsilon} \alpha(f(x';\theta),y) = \mathbb{E}_{(x, y)} \alpha(f(x;\theta),y)
\end{equation}
which is usually optimized through maximizing: 
% the following: 
\begin{equation}
   \mathbb{E}_{(x, y)} \min_{x':d(x', x) \le \epsilon} \alpha(f(x';\theta),y)
\end{equation}
where $\alpha$ denotes the function evaluating prediction accuracy. In the case of classification, $\alpha(f(x; \theta), y)$ yields 1 if the prediction $f(x; \theta)$ equals ground-truth label $y$, 0 otherwise. The distance metric $d(\dot, \dot)$ is usually approximated by $L_0$, $L_2$ or $L_\infty$ to measure the visual dissimilarity of original image $x$ and the perturbed image $x'$. Despite the change to the input is small, the community have found a class of methods that can easily manipulate model's predictions by introducing visually imperceptible perturbations in images \cite{szegedy2013intriguing,  goodfellow2014explaining, moosavi2016deepfool}. 
From the optimization standpoint, it is achieved by maximizing the loss of the model on the input \citep{madry2017towards}:
\begin{equation}
   \max_{\delta} \ l(f(x + \delta;\theta), y) \;\; \textnormal{s.t.} \;\; d(x + \delta, x)  < \epsilon \label{eq:optim}
\end{equation}
where $l(\cdot, \cdot)$ denotes the loss function (\eg, cross entropy loss) for training the model $f$ parameterized by $\theta$. 
While these attack methods are powerful, 
they usually 
require some degrees of knowledge about the target model $f$ (\eg, the gradient). 
Arguably, for many real-world settings, 
% these assumptions may be unrealistic. 
such knowledge is not available, 
and we can only expect less availability 
of such knowledge on 
% This is all the more so in 
FL applications trained and deployed by service providers. 
On the other hand, 
% Embracing the hypothetical scenarios where 
the hostile attacker having access to some but limited amount of users' data is a much more realistic scenario.
Thus, we propose the following assumption for practical attack in FL: 
% \begin{assumptionp}{}
given the data of $n$ malicious users $D_m = \bigcup_{i=1}^{n} D_i$ where $D_i = \{(x_k, y_k)| k = 1, \cdots, m_i\}^{(i)}$ contains $m_i$ data points, we aim to acquire a transferable perturbation $\delta$ by maximizing the same objective as in Equation \ref{eq:optim} but with a surrogate model $f'$ parameterized by $\theta'$ trained by $D_m$:
\begin{equation}
   \delta = \mathop{\arg\min}_{\delta} \ l(f'(x + \delta;\theta'), y) \;\; \textnormal{s.t.} \;\; d(x + \delta, x)  < \epsilon 
\end{equation}
We hope to test whether this $\delta$ can be used to deceive the target model $f$ as well.
% \end{assumptionp}
\subsection{The Security and Robustness of Federated Learning}
% FL provides one of the most promising solutions to take advantage of the large amount of distributed data collected from user-end without violating privacy requirements. However,  the loose organization and its invisibility to local data makes it more vulnerable to the various attacks.
\textbf{Poisoning and Backdoor Attack.}
Poisoning attack including data \cite{biggio2012poisoning} and model poisoning attack \cite{fang2020local} aims to maximize the classification error of global model via malicious data injection or local model parameter manipulation on compromised client devices. Backdoor attack, instead, aims to inject a malicious task into the existing model while retaining the accuracy of the actual task \cite{bagdasaryan2020backdoor, sun2019can}. \cite{chen2017targeted} propose the model replacement to replace the global model with a backdoored model stealthily. \cite{fung2018mitigating} introduce label-flipping to backdoor the federated model while \cite{xie2019dba} uses GANs to attack the global model. Boosting weights and including stealth into the adversarial objective also proves to be effective to backdoor \cite{bhagoji2019analyzing}. To defend against these attacks, various anomaly detection based methods have been proposed. One of the earliest is the Byzantine-tolerant (or Byzantine-resistant) aggregation \cite{shejwalkar2021manipulating} such as Krum, MultiKrum \cite{blanchard2017machine}, Bulyan \cite{guerraoui2018hidden}, Trimmed-mean and Median \cite{yin2018byzantine}, which focuses mainly on geometric distance between the hostile gradients and benign ones. \cite{shen2016auror} uses clustering to distinguish the malicious updates from a collaborate of clients while \cite{fang2020local} proposes Error Rate and Loss based Rejection which rejects updates that has large influence to either error rate or model loss on the validation set. \cite{li2020learning, kieu2019outlier} learns another model to detect malicious updates in the spectral domain. \cite{zawad2021curse} discovers that the data heterogeneity of FL largely impacts the robustness and attack performance of backdoor attack. Knowledge distilliation and prunning is also proven effective to prevent these attacks \cite{li2019fedmd, liu2018fine}.

\textbf{Transfer Attack.}
% Adversarial attack refers to a type approach that generates imperceptible perturbations which leads to mis-classification with high confidence \cite{szegedy2013intriguing, biggio2013evasion}. The community has discovered various types of powerful attack methods such as FGSM \cite{goodfellow2014explaining}, PGD \cite{madry2017towards}, deepfool \cite{moosavi2016deepfool} and many others \cite{carlini2019evaluating, xiao2018generating, dong2018boosting}. Despite that machine learning models are highly susceptible to adversarial examples, these attacks require various knowledge of the model to ensure a successful attack, which is impractical in real-world scenarios. Consequently, black-box attack is introduced which can be divided into query-based and transfer-based attack. Query-based attack requires queries to the target model and treat the prediction as the ground-truth label forming the initial training set to train the surrogate model \cite{papernot2017practical}. Augmentation and regularization are leveraged to further improve the attack \cite{guo2019simple, wang2021delving}. Despite the queries can help the source model to learn a decision boundary similar to one of the target model, the requirement for query make it impractical to attack systems with access limit. 
Transfer-based adversarial attack leverages the full training set used by the target model to train a surrogate model \cite{zhou2018transferable}. The condition for transfer attack in practice is also difficult to achieve since it's even more difficult or costly and laborsome to access the original training set or collecting a similar new one, especially in FL where data privacy are carefully protected. Another research perspective is the mechanism behind the black-box attack. Black-box attack builds upon an intriguing discovery that adversarial examples are higher transferable even between models of different architectures \cite{szegedy2013intriguing, goodfellow2014explaining}. This transferability can be partly explained by the similarity between the source and target models. \cite{goodfellow2014explaining, liu2016delving} shows that adversarial perturbations are highly aligned with the weight vectors of a model and that different models learn similar decision boundaries when trained to perform the same task. \cite{tramer2017space} discovers that adversarial examples span a contiguous subspace of large dimensionality and the shared subspace of two models enables the transferability. While \cite{ilyas2019adversarial} shows that adversarial perturbations are non-robust feature captured by the model, \cite{waseda2023closer} uses this theory to explain why different mistakes exist in the transfer attack. \cite{demontis2019adversarial} demonstrates that a similar gradient of source and target model and a low variance of loss landscapes leads to a higher possibility to transfer attack. We highlight the key differences and significance of our setting compared with others.

\textbf{Key Difference 1:} 
Different from query-based or transfer-based black-box attack, we assume the malicious clients possess the data themselves, impacting the target model during training and attack during inference. We also present a comparison of our attack setting and the query-based attack in Appendix \ref{appendix:comparision_query}. Note that our attack setting doesn't contradict with the query-based attack. In fact, we can perform with both if the FL system allows a certain number of queries, which we leave to future works to explore.

\textbf{Key Difference 2:} 
Poisoning attack or backdoor attack manipulates the parameters update during target model training which can be defended by anomaly detection. Moreover, in practice, despite clients preserving the training data locally, the training procedure and communication with the server are highly encapsulated and encrypted with secret keys, which is even more unrealistic and laborsome to manipulate. Our attack setting circumvents this risk since no hostile action is performed during the training but successfully boost the attack possibility during inference time. 

\textbf{Significance :}  Besides the potential data leakage by malicious participants, we also emphasize that despite, ideally, each participant having access to the global model, in real-world applications (e.g. Gboard \cite{hard2018federated}), the infrastructure provider will impose additional protection such as encryption or encapsulation over the local training. For instance, Gboard from Google provides the next-word prediction with FL, which requires users to install an app to participate. For an adversary, it's impractical to obtain the global model without breaking or hacking the app or hijacking and decrypting the communication, despite all the things happening "locally". We believe this is much more difficult and laborsome than our setting which significantly boosts the transferability by simply acting as a benign.

==> sections/table1.tex <==
\begin{table}[t]
\footnotesize  
\centering
\caption{Centralized and federated model under white-box attack.}

\setlength{\tabcolsep}{0.4mm}{
\begin{tabular}{cccccc}
\hline
 \multirow{2}{*}{Paradigm} & \multirow{2}{*}{Architecture} & \multicolumn{2}{c}{same-acc} & \multicolumn{2}{c}{same-epoch} \\
& & Acc & Adv.Acc & Acc & Adv.Acc \\
\hline
\multirow{4}{*}{centralized} & R50       & 90.20 & 0.01  & 95.24 & 0.40      \\
                             & R50 (adv) & 81.23 & 23.27 & 89.46 & 46.09    \\
                             & CNN  & 75.06 & 1.24  & 82.41  & 0.35      \\
                             & CNN (adv) & 73.15 & 20.89 & 76.78 & 28.92    \\
\hline
\multirow{4}{*}{federated} & R50         & 90.29 & 0.05 & 92.31 & 0.02 \\
                           & R50 (adv)   & 80.05 & 36.44 & 81.05 & 39.11  \\
                           & CNN  & 75.09  & 3.68  & 76.83 & 3.98   \\
                           & CNN (adv) & 72.85 & 25.5 & 72.87 & 24.35    \\
\hline
\end{tabular}
}
\label{tab:baseline}
\end{table}

==> sections/table2.tex <==

\begin{table}[t]
\footnotesize 
\centering
\caption{T.Rate and transfer accuracy of PGD attack between pairs of models using various training paradigms. The row and column denote the source and target model respectively. For each cell, the left is the transfer accuracy and the right is the T.Rate.}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ccccccc}
\hline
 & & federated & centralized \\
\hline
\multirow{2}{*}{R50}& federated   & 0.15 / 99.83 & 2.01 / 97.67   \\
&centralized & 24.28 / 71.94 & 7.41 / 91.48  \\

\hline
\multirow{2}{*}{CNN}& federated   & 19.31 / 76.32 & 21.59 / 71.84   \\
&centralized & 30.57 / 56.59 & 22.62 / 68.19  \\
\hline
\end{tabular}
}
\label{tab:transfer_robustness}
\end{table}

==> sections/table_combined.tex <==
\begin{minipage}{\textwidth}
\begin{minipage}[t]{0.49\textwidth}
\makeatletter\def\@captype{table}
\footnotesize  
\centering
\caption{Centralized and federated model under white-box attack.}
\setlength{\tabcolsep}{0.4mm}{
\begin{tabular}{cccccc}
\hline
 \multirow{2}{*}{Paradigm} & \multirow{2}{*}{Architecture} & \multicolumn{2}{c}{same-acc} & \multicolumn{2}{c}{regular} \\
& & Acc & Adv.A & Acc & Adv.A \\
\hline
\multirow{4}{*}{centralized} & R50       & 90.20 & 0.01  & 95.24 & 0.40      \\
                             & R50 (adv) & 81.23 & 23.27 & 89.46 & 46.09    \\
                             & CNN  & 75.06 & 1.24  & 82.41  & 0.35      \\
                             & CNN (adv) & 73.15 & 20.89 & 76.78 & 28.92    \\
\hline
\multirow{4}{*}{federated} & R50         & 90.29 & 0.05 & 92.31 & 0.02 \\
                           & R50 (adv)   & 80.05 & 36.44 & 81.05 & 39.11  \\
                           & CNN  & 75.09  & 3.68  & 76.83 & 3.98   \\
                           & CNN (adv) & 72.85 & 25.5 & 72.87 & 24.35    \\
\hline
\end{tabular}
}
\label{tab:baseline}
\end{minipage}
\begin{minipage}[t]{0.49\textwidth}
\makeatletter\def\@captype{table}
\footnotesize 
\centering
\caption{T.Rate and transfer accuracy of PGD attack between pairs of models using various training paradigms. The row and column denote the source and target model respectively. For each cell, the left is the transfer accuracy and the right is the T.Rate.}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ccccccc}
\hline
 & & federated & centralized \\
\hline
\multirow{2}{*}{R50}& federated   & 0.15 / 99.83 & 2.01 / 97.67   \\
&centralized & 24.28 / 71.94 & 7.41 / 91.48  \\

\hline
\multirow{2}{*}{CNN}& federated   & 19.31 / 76.32 & 21.59 / 71.84   \\
&centralized & 30.57 / 56.59 & 22.62 / 68.19  \\
\hline
\end{tabular}
}
\label{tab:transfer_robustness}
\end{minipage}
\end{minipage}

